SkiNet, A Petri Net Generation Tool for the Verification of Skillset-based Autonomous Systems

The need for high-level autonomy and robustness of autonomous systems for missions in dynamic and remote environment has pushed developers to come up with new software architectures. A common architecture style is to summarize the capabilities of the robotic system into elementary actions, called skills, on top of which a skill management layer is implemented to structure, test and control the functional layer. However, current available verification tools only provide either mission-specific verification or verification on a model that does not replicate the actual execution of the system, which makes it difficult to ensure its robustness to unexpected events. To that end, a tool, SkiNet, has been developed to transform the skill-based architecture of a system into a Petri net modeling the state-machine behaviors of the skills and the resources they handle. The Petri net allows the use of model-checking, such as Linear Temporal Logic (LTL) or Computational Tree Logic (CTL), for the user to analyze and verify the model of the system.

==> eptcsdata.tex <==
\providecommand{\firstpage}{120}
\providecommand{\publicationstatus}{M. Luckcuck and M. Farrell; M. Autili, L. Berardinelli,\\ A. Bucaioni and C. Pompilio (Eds.):\\
Formal Methods for Autonomous Systems and \\
Automated and verifiable Software sYstem DEvelopment \\
EPTCS 371, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.371.9}{10.4204/EPTCS.371.9}}
\pdfoutput=1

